ReasonBERT: Pre-trained to Reason with Distant Supervision

We present ReasonBert, a pre-training method that augments language models with the ability to reason over long-range relations and multiple, possibly hybrid contexts. Unlike existing pre-training methods that only harvest learning signals from local contexts of naturally occurring texts, we propose a generalized notion of distant supervision to automatically connect multiple pieces of text and tables to create pre-training examples that require long-range reasoning. Different types of reasoning are simulated, including intersecting multiple pieces of evidence, bridging from one piece of evidence to another, and detecting unanswerable cases. We conduct a comprehensive evaluation on a variety of extractive question answering datasets ranging from single-hop to multi-hop and from text-only to table-only to hybrid that require various reasoning capabilities and show that ReasonBert achieves remarkable improvement over an array of strong baselines. Few-shot experiments further demonstrate that our pre-training method substantially improves sample efficiency.

==> sections/bg.tex <==
\section{Background}
\subsection{Problem Setting}
\label{sec:problem}
\st{Our work is inspired by the extractive question answering task, here we define the task as follows.} \hs{[Similar as intro, start with drawbacks of pre-training and goals we want to achieve, and then] inspired by the formulation of extractive QA, we develop this pretraining method. Now let us first clarify the extractive QA task:}

Given a question $q$ and provided evidence $E$, the QA model $p_\theta(a|q,E)$ aims to select a contiguous span $a$ from $E$ that answers the question, or output "\textit{No Answer}" if $E$ is not sufficient to answer the question. 
Early QA datasets like SQuAD contain mostly simple single-hop questions that use only a single context as input and do not require deep comprehension and reasoning. 

Recently, people have studied more challenging QA tasks, including multi-hop QA, where the model needs to first filter out irrelevant information from a set of contexts, and then combine multiple disjoint pieces of evidence to find the answer, and hybrid QA, where the evidences include both unstructured text and structured tables. We design our approach to benefit all these settings, and conduct comprehensive experiments with a wide range of QA benchmarks under both few-shot and fully supervised scenarios.

\subsection{Base QA Model}
\label{sec:baseqa}
\nop{I think I understand what the relationship between C and E is, but that seems not clear from the writing.} We first consider a base QA model $p_\theta(s,e|q,E)$, that takes as input the question $q$, the selected evidence $E$, and outputs $s,e$ which are the start, end location of the answer in $E$. Inspired by previous works, we design the base QA model as a sequence encoder, with answer selection headers on top. More specifically, we first concatenate $q,E$ and add special tokens to form the input sequence as $[\texttt{[CLS]},q,\texttt{[QUESTION]},\texttt{[SEP]},E]$, and get the contextualized input representation $\mathbf{x}$ with the encoder. To extract the answer from $E$, we predict the answer span's start and end position $s, e$ as follows:

\begin{equation}
\begin{aligned}
P(s=i \mid q, E)&=\frac{\exp \left(\mathbf{x}_{i}^{\top} \mathbf{S} \mathbf{x}_{q}\right)}{\sum_{j} \exp \left(\mathbf{x}_{j}^{\top} \mathbf{S} \mathbf{x}_{q}\right)} \\
P(e=i \mid q, E)&=\frac{\exp \left(\mathbf{x}_{i}^{\top} \mathbf{E} \mathbf{x}_{q}\right)}{\sum_{j} \exp \left(\mathbf{x}_{j}^{\top} \mathbf{E} \mathbf{x}_{q}\right)}
\end{aligned}
\label{eqn:selection}
\end{equation}

Here $\mathbf{S}, \mathbf{E}$ are trainable parameters of the the answer selection headers, which extract start and end query vectors using the representation $\mathbf{x}_{q}$ of special token \texttt{[QUESTION]}. If no answer can be found in the provided evidence, we set $s,e$ to point to the \texttt{[CLS]} token. \hs{I feel how the encoder representations from Section 4.1 are used in this base QA model or how the pre-trained architecture connects with the base model is not clear yet.}

The loss is then calculated as:
\begin{equation}
    L = - \mathrm{log}P(s|q,E)- \mathrm{log}P(e|q,E)
\end{equation}

At inference time we score all the start, end locations and rank all spans $(s,e)$ by $g(s,e|q,E)$:

\begin{align}
    f_\mathbf{start} = \mathbf{x}_{i}^{\top} \mathbf{S} \mathbf{x}_{q}&,\ \ \ \ f_\mathbf{end} = \mathbf{x}_{i}^{\top} \mathbf{E} \mathbf{x}_{q} \\
    g(s,e|q,E)&= f_\mathbf{start}(s|q,E)\\
    &+f_\mathbf{end}(e|q,E) \nonumber\\
    &-f_\mathbf{start}(\texttt{[CLS]}|q,E) \nonumber\\
    &-f_\mathbf{end}(\texttt{[CLS]}|q,E) \nonumber
\end{align}


In this work, we aim to directly pretrain such a QA model with unlabeled Wikipedia corpus. 

==> sections/intro.tex <==
\begin{abstract}
\hs{Candidate titles:
\\ 0. Learning to Fuse for Question Answering with Distant-Supervised Pretraining (from Xiang)
\\1. Distantly Supervised Pretraining for (Multi-hop, Hybrid) Question Answering\\2. Distantly Supervised Pretraining to Reason for (Multi-hop, Hybrid) Question Answering}

\hs{I feel `learning to fuse' seems to imply we will have a `retrieval' step in pretraining.}

With advanced neural models achieving near-human performance on simple question answering (QA) benchmarks, there is an increasing attention on complex question answering that requires a model to not only reason over multiple contexts, but also to handle heterogeneous data sources like texts and tables. However, even with large pretrained language models, training a QA system still requires a massive amount of supervised data, which is hard to obtain for complex QA tasks. To address this, we propose to pretrain a QA model over query-evidence pairs collected from unlabeled Wikipedia corpus via distant supervision. Given a query sentence with entities masked to simulate question and answers, we find sentences or tables that contain the same entities to serve as evidences. We then pretrain the model to recover the masked entities from the evidences, so it learns to fuse information from multiple heterogeneous sources. The resulting model obtains significant improvements on various complex QA benchmarks including HotpotQA and HybridQA. Further experiments under few-learning setting also show that our model is sample-efficient, achieving competent performance with much less supervised training examples.
\end{abstract}
\section{Introduction}
\begin{figure*}[ht]
    \centering
    \includegraphics[width=\linewidth]{figures/example.jpeg}
    \vspace{-2em}
    \caption{Examples of the pretraining data acquired by distant supervision, best view with color. Our pretraining data covers a wide range of topics with both textual and tabular data as evidence. We encourage the model to learn deep reasoning by combining multiple evidences to simulate reasoning chains. For example, in the second and third example, the green entities act as bridge which is needed in order to infer other entities. \hs{For the third example, should we highlight `awaken the guardian' in the query text? The `Halloween' in the first example is highlighted. do we have another example showing a different reasoning type (e.g., intersection type)? The last two examples have the same bridge type.}
    \ww{+1 to highlighting `Awaken the Guardian'.  Also, is there an example where we mask entities in a table as [QUESTION], and use multiple texts as supporting evidence to recover the entity, or is that not part of goal for this work?}}
    \vspace{-1em}
    \label{fig:example}
\end{figure*}
Great progress has been made in building question answering (QA) systems in the past few years \cite{XX}. With the help from large-scale pretrained language models, well-designed neural models have achieved or even exceeded human performance on simple single-hop QA benchmarks like SQuAD. In light of this, recently more and more work has studied more challenging complex QA \hs{should we be more specific and directly say `multi-hop?'} tasks. Unlike simple QA where the model can answer a question based on a single sentence or document, complex QA considers a more realistic setting where the model needs to \hs{reason over multiple pieces of information that can range from unstructured to structured.}%fuse information from multiple sources and understand different format of evidence including both unstructured data like text and structured data like tables and lists. 

This poses many new challenges to existing QA systems. First, the conventional method to train a QA model requires large-scale supervised data, which is significantly more costly to acquire for complex QA, as the annotator needs to inspect multiple disjoint pieces of evidence and construct a reasonable reasoning chain. Second, state-of-the-art QA models rely heavily on pretrained language models (LMs). However, pretraining objectives like masked language modeling (MLM) do not necessarily teach the model to do deep reasoning across multiple contexts, since the input is usually contiguous sentences and many of the masked tokens can be recovered from local cues.

In this work, we aim to address the challenge by pretraining the QA model using query-evidence pairs collected from unlabeled Wikipedia corpus via distant supervision. The intuition is that any sentence (or table) that contains the same pair of entities is likely to express the relation between the entities in some way \ww{``the same way''?}, and can be used to support it. In other words, given a query sentence with one of the entities masked, another sentence (or table) that contains the same pair of entity can be used as evidence to recover the missing entity. In light of this, we propose a novel pretraining method: \textit{grounded span selection}. We simulate the QA task by masking certain entities in a query sentence, and pretrain the model to recover them based on the given evidences. We adopt a standard QA model that uses a pretrained encoder with answer selection layers on top. At pretraining phase, we replace the masked entities with \texttt{[QUESTION]} tokens, and use their contextualized representation to select the missing entities from the provided evidences. During fine-tuning, we simply append the \texttt{[QUESTION]} token to the question, and select the answer span the same way as in pretraining. To encourage the model to conduct deep reasoning, we include multiple evidences in the input, and scatter the masked entities among them to mimic different types of reasoning chains. To enable the model to handle both structured and unstructured data, we consider both tables and text as evidence, and adopt the recent structure aware transformer from TAPAS with extra column and row selection objectives to help the model understand table structure.

We evaluate our pretraining approach on three datasets: HotpotQA, a text-only multi-hop QA dataset; NQTables, a subset of the Natural Questions dataset where the answer can be found in tables; and HybridQA, a heterogeneous multi-hop QA dataset that requires reason over both tables and text. Experimental results show that our method obtains significant gain over existing pretraining approaches like RoBERTa. With a simple QA model architecture, our method achieves the same or even better performance compared with more sophisticated state-of-the-art models.

Moreover, the consistency between pretraining and fine-tuning makes our model an efficient few-shot learner. In addition to the three datasets above, we also include eight datasets of different domains from the MRQA benchmark for evaluation under few-shot learning setting. The results show that our model substantially outperforms the baselines and achieves competent performance with much less supervised training examples.

==> sections/intro_v1.tex <==
\begin{abstract}

\nop{
\hs{Candidate titles:
\\00. Distantly Supervised Pretraining to Reason with Comprehensive Evaluation on Extractive QA (Huan: to tone down `reason,' I removed it from the current title.)
\\ 0. Learning to Fuse for Question Answering with Distant-Supervised Pretraining (from Xiang)
\\1. Distantly Supervised Pretraining for (Multi-hop, Hybrid) Question Answering\\2. Distantly Supervised Pretraining to Reason for (Multi-hop, Hybrid) Question Answering
\\2. Pretrained to Reason via Distant Supervision}

\hs{I feel `learning to fuse' seems to imply we will have a `retrieval' step in pretraining.}
\add{other titles: XX: Distantly Supervised Pretraining. Here some choices of XX: QABert; ReasonBert }
}

We present \ours, a pretraining method that encourages the model to explicitly reason over multiple contexts, ranging from unstructured text to structured tables. Inspired by question answering (QA), instead of randomly masking and predicting tokens on a single paragraph, we pretrain the model to extract masked answer spans from relevant evidence. We employ distant supervision to collect query-evidence pairs from an unlabeled Wikipedia corpus and thus obviate the need of a separate evidence retriever or question generator. Given a query sentence with entities masked to simulate question and answers, we find sentences or tables that contain the same entities to serve as evidences. To empower the model to conduct deep reasoning, we mimic different types of reasoning chains by masking multiple entities, including unanswerable ones, and simultaneously extracting them from disjoint pieces of evidences. The resulting model obtains significant improvements on various QA benchmarks that requires complex reasoning, including HotpotQA and HybridQA. Further experiments under few-learning setting also show that the learned reasoning ability can be efficiently transferred to downstream task, achieving competent performance with much less supervised training examples.
\end{abstract}
\section{Introduction}
\begin{figure*}[ht]
    \centering
    \includegraphics[width=\linewidth]{figures/example_v1.png}
    \vspace{-2em}
    \caption{Examples of our pretraining data acquired via distant supervision (DS). Best viewed in color. Our pretraining data covers a wide range of topics with both textual and tabular evidences. For each query sentence, we first select two pairs of entities (underlined) to find evidences with DS. We then randomly mask one entity from each selected pair and the task is to recover it by selecting from the evidence (the two selected pairs may share a common entity, and it is possible this entity is masked). We additionally mask one entity that does not exist in the evidences to simulate unanswerable cases. Our way of collecting pretraining data allows us to simulate different reasoning chains and encourage the model to conduct deep reasoning. In the first example, the model need to check multiple properties, and find \textit{the \textbf{beach soccer} competition that is established in \textbf{1998}}. In the second example, the model is asked \textit{what is the type of the band that releases \textbf{Awaken the Guardian}}, for which it needs to first infer the bridging entity \textbf{Fates Warning}. \nop{For the third example, should we highlight `awaken the guardian' in the query text? The `Halloween' in the first example is highlighted. do we have another example showing a different reasoning type (e.g., intersection type)? The last two examples have the same bridge type.}\nop{+1 to highlighting `Awaken the Guardian'.  Also, is there an example where we mask entities in a table as [QUESTION], and use multiple texts as supporting evidence to recover the entity, or is that not part of goal for this work?}\nop{we only use sentences as query, which simulates questions. For \textit{Awaken the Guardian}, it is not one of the sampled entities. At each round we only sample two entity pairs from the query, and mask from them. However, there may exists other common entities, should we highlight them as well?}\nop{perhaps no, but this orange text might be put in footnote. Also, we might need to make the figure a bit prettier.} \nop{the last two examples seem problematic; 1998 also appears in the left paragraph and you don't need the two evidences to infer the answer in the last example too.}}
    \vspace{-1em}
    \label{fig:example}
\end{figure*}

Recent advances in language model pretraining have remarkably transformed the landscape of natural language processing \cite{XX}. The most prevalent approaches are variants of masked language models (MLMs) \cite{XX}, which are trained to reconstruct corrupted input sequences sampled from unlabeled text corpora. It has been shown that MLMs can achieve state-of-the-art results on a wide range of NLP tasks. %\hs{After reading the next paragraph, people might argue these two tasks, especially `relation extraction' also requires reasoning..}
\hs{However, MLMs tend to implicitly memorize the learned world knowledge in the parameters of the underlying neural network and make shallow predictions based on local cues.\st{fine-tuning a pretrained language model for tasks like question answering still requires massive supervised data.}}For example, ... \add{give an example of memorizing world knowledge here; check REALM paper}  %\hs{we only have few-shot learning settings for simple QA, right? I wonder if we should use `the need for training data' as an argument.}
\nop{However, fine-tuning a pretrained language model for tasks like question answering still requires massive supervised data. One possible explanation is that MLMs tend to implicitly memorize the learned knowledge in the parameters of the neural network, and make shallow predictions based on local cues. While for tasks like QA, it is important for the model to capture long range relations and explicitly reason over the given contexts.}

To encourage a model to capture long-range relations and explicitly reason over multiple contexts, we present \ours, a pretraining method that defines a distantly supervised task to augment language model pretraining.  Unlike exiting pretraining objectives which predict masked individual tokens or spans in a single contiguous paragraph, \ours\ masks entities in a query sentence and pretrains a model to recover them by reasoning over relevant evidences. %assuming we can obtain $<$query sentence, evidence$>$ pairs.

\nop{Inspired by the QA task, which has become an important testbed for evaluating how well NLP models can understand and reason with languages \cite{xx}, we pretrain the model to answer a question based on given evidences. In this work, we simulate questions by masking entities in a query sentence and treat the masked entities as answers, and pretrain the model to extract the answers from relevant evidences.}

\nop{We present \ours, a pretraining method inspired by QA that encourages the model to learn to explicitly reason over multiple contexts, ranging from unstructured text to structured tables. Recently, QA has become an important testbed for evaluating how well NLP models can understand and reason with languages, where the model needs to answer a question based on given evidences. In this work, we simulate questions by masking entities in a query sentence as answers, and pretrain the model to extract the answers from relevant evidences.}

One challenge in developing \ours\ lies in how to create a large set of query-evidence pairs for pretraining.\nop{\xd{Unlike existing works that use a separate evidence retriever \cite{xx} or question generator \cite{xx},} We draw inspiration from the idea of \textit{distant supervision} \cite{XX}.}
%To collect query-evidence pairs from an unlabeled corpus that can contain both texts and tables, we borrow the idea of distant supervision. 
We draw inspiration from the idea of \textit{distant supervision}, which assumes that if two entities hold a certain relation, any sentence (or \xd{record in table}\nop{rows?}) that contains them expresses the relation in some way and can be used as supporting evidence. Therefore, given a query sentence with one of the entities masked, another sentence (or \xd{record in table}\nop{row?}) that contains the same pair of entities can be used as evidence to recover the masked entity. \add{Moreover, to encourage a model to conduct deep reasoning, we collect multiple evidences that shall be jointly used to recover the masked entities in the query sentence, and scatter the answers among them to mimic different types of reasoning chains {(See Figure \ref{fig:example})}. In addition, we enable a model to handle hybrid evidences that include structured tables and unstructured text.} %\hs{[a few sentences on how the dataset is eventually collected.. especially those examples in Figure 1 that need complex reasoning.]} 

%\hs{rephrase this paragraph by posing `grounded span selection' objective and why it helps?} 
Once the query-evidence pairs are collected, in the pretraining phase, we replace the masked entities in a query sentence with \texttt{[QUESTION]} tokens, and use their contextualized representation to reason about the answer spans from the provided evidences. We adopt the encoders in XX and XX to represent the concatenated query sentence and textual evidences, with question-aware answer extraction layers on top. When tabular evidences are present, we use the recent structure-aware transformer from TAPAS \cite{XX} as the encoder to help capture the table structure.
\nop{When finetuning for QA tasks, we append the \texttt{[QUESTION]} token to the question and get contextualized representations with the pretrained encoder. To encourage the model to conduct deep reasoning, we include multiple evidences in the input, and scatter the answers among them to mimic different types of reasoning chains {(See Figure \ref{XX})}. To enable our model to handle both structured and unstructured data, we consider both tables and texts as evidence, and adopt the recent structure-aware transformer from TAPAS \cite{XX} to help the model understand table structure.
}

We choose to evaluate \ours\ on the extractive QA task, which is arguably the most representative task that requires reasoning about world knowledge. When finetuning the models \add{pretrained by \ours\} for extractive QA, we append the \texttt{[QUESTION]} token to the question and get its contextualized representation from the pretrained encoder.  We conduct a comprehensive evaluation using a variety of datasets under both few-shot and fully-supervised settings: MRQA \cite{XX}, a text-only single-hop QA benchmark including six datasets from different domains; HotpotQA \cite{XX}, a text-only multi-hop QA dataset; NQTables, a subset of the Natural Questions dataset \cite{XX} where answers can be found in tables; and HybridQA \cite{XX}, a hybrid multi-hop QA dataset that requires reasoning over both tables and text. Under the few-shot setting, \ours\ substantially outperforms the baselines in all datasets, demonstrating that the learned reasoning ability {during pretraining} can be easily transferred to downstream QA tasks and generalize well across domains. Under the fully-supervised setting, \ours\ obtains substantial gains in multi-hop and hybrid QA datasets compared with baselines. {Despite built on top of a simpler model architecture}, \ours\ achieves similar or better performance compared with more sophisticated state-of-the-art models \add{for each dataset}.

==> sections/model.tex <==
\section{Pretraining}
\subsection{Encoder}
In this work, we consider both textual and tabular evidences. For the text-only setting, we adopt the standard transformer encoder in BERT \cite{devlin-etal-2019-bert}. For settings where the input contains structured data, we use the transformer variant introduced in TAPAS \cite{herzig-etal-2020-tapas}, which uses extra token-type embeddings \nop{like row and column embeddings}{(indicating the row/column position of a token)} to model the table structure.

\subsection{Grounded Span Selection} 
We propose a novel \hs{When I read to this part, I somehow feel it is a bit straigtforward and there is no surprise. How to revise the writing to avoid the impression? how about starting with the red sentence?} apporach to pretrain question answering using unlabeled text and tables: \textit{grounded span selection}. 

\add{Inspired by the extractive QA task, we propose a new pretraining objective, \textit{grounded span selection}, which can advance reasoning capabilities of the pretrained model.}

Given a sample collected for pretraining as described in Section \ref{sec:data_generation}. We replace masked entities $\mathcal{A}=\{a_1,a_2,\dots,a_n\}$ in the query sentence $q$ with special \texttt{[QUESTION]} tokens. The task is then to recover these masked entities\nop{as we discussed earlier, the `grounding' notion is a bit strange. Why don't we simply say extracting answers from $E$?} from the given evidence $E$. More specifically, we use the base QA model described in Section \ref{sec:baseqa} \hs{how about we remove the description in the earlier description and direction describe how a typical QA model works..} to predict the start and end location of the masked entity $a_i$ in $E$ \hs{This is what we mean by `grounded,' right?}. Since we have multiple "answers" masked with \texttt{[QUESTION]} tokens, a fixed query vector $\mathbf{x}_q$ as in Eqn. \ref{eqn:selection} is inapplicable. Instead, for each $a_i$, we use the representation $\mathbf{x}_{a_i}$ of the associated \texttt{[QUESTION]} token to replace $\mathbf{x}_q$ as a dynamic query vector. The \textit{grounded span selection} loss is then calculated as follows:
\begin{equation}\small{
    L_{GSS} = -\sum_{a_i \in \mathcal{A}} \left(\mathrm{log}P\left(s_{a_i}|q,E\right)+ \mathrm{log}P\left(e_{a_i}|q,E\right)\right)
}\end{equation}

The \textit{grounded span selection} objective can help the encoder learn better contextualized representations during pretraining, \nop{for multi-hop QA in the following ways}due to the following reasons: (1) Instead of predicting individual tokens as in the masked language modeling objective, we directly pretrain span selection, which is consistent with the downstream QA model. \hs{should we also compare with other span prediction objectives like the one in SpanBert to better stress what we mean by `grounded' span selection? in other words, what is `ungrounded' like?} (2) Unlike previous works \cite{XX} that use single contiguous paragraph as context, where the model may focus on local cues, we encourage the model to do long-range contextualization by including both query and evidence as input, which can come from different passages and recover the masked entity \add{by} grounding on the evidence. (3) To improve the model's ability of doing deep reasoning across multiple pieces of evidence, we include two disjoint pieces of evidence in a single sample, and scatter the answer entities among them to mimic different types of reasoning chains. (4) To cope with unanswerable questions in QA datasets, and the need to filter out irrelevant evidences in multi-hop QA, we also mask entities that do not appear in $E$, in which case the model is asked to select the special \texttt{[CLS]} token. \hs{perhaps revise this part so that it does not sound like the model is tailored for QA, but QA is one of the tasks the model can better serve?}

\nop{
\subsection{Table Cell Selection}
To help the model learn to reason over tables, we also include a cell selection objective. In addition to predict the start and end location of the target entity, the model is taught to select the row and column by aggregating information from all cells in the that row or column. More specifically, we calculate the probability of target $a$ belongs to row $r_j$ as follows:
\begin{equation}\small{
\begin{aligned}
    S_{cell}&=\mathrm{mean}_{x_i \in cell}\left(\mathbf{x}_{i}^{\top} \mathbf{R} \mathbf{x}_{a}\right)\\
    P(r_a=j \mid q, E)&=\frac{\exp \left(\max_{cell \in r_j}S_{cell}\right)}{\sum_{k} \exp \left(\max_{cell \in r_k}S_{cell}\right)}
\end{aligned}
}\end{equation}
Here $\mathbf{R}$ is the weight matrix of row selection header, and the column selection probability is calculated similarly with another column selection header. We first score each cell by averaging over all tokens in that cell. We then do a max pooling over all cells in the row or column so the model can focus on the strongest signal, for example the column header. The \textit{cell selection} loss is then calculated as follows:
\begin{equation}\small{
    L_{CS} = -\sum_{a_i \in \mathcal{A}} \left(\mathrm{log}P\left(r_{a_i}|q,E\right)+ \mathrm{log}P\left(c_{a_i}|q,E\right)\right)
}\end{equation}
}

\subsection{Final Objective}
We also include the \textit{masked language modeling} (MLM) objective in pretraining to leverage other tokens in the input that are not entities. In particular, we randomly mask tokens that are not part of an entity or tokens in the header row for tables, and use a MLM header to recover it. Following the default parameter from BERT, here we use a masking probability of 15\%.

The final loss for pretraining is the sum of \textit{grounded span selection} loss and \textit{masked language modeling} loss for text-only inputs. %plus additional \textit{table cell selection} loss for hybrid inputs with tables.

\subsection{Pretraining Details}
We set the max length of query sentences to 100 tokens and max length of each evidence to 200 if there are two evidences or 400 if there is only one. For textual evidences, we include the neighbouring sentences from the same paragraph as extra context for the selected evidence sentence and clip to the max evidence length. For tabular evidences, we take a snippet of the original table, and truncate the cells to 20 tokens. We always keep the first row and column in the table, as they tend to contain important information such as headers and subject entities. Based on the selected entity pair, we sample up to 5 columns and include as many rows as possible until reaching the budget.

We initialize {our encoder} with RoBERTa-base \cite{XX} for the text part\nop{-only setting}, and TAPAS-base \cite{XX} for the table part\nop{hybrid setting}. We train \ours\ using AdamW \cite{} for 10 epochs with batches of 256 sequences of length 512; this is approximately 290k steps with text-only data, and 120k steps with hybrid data. We base our implementation on Huggingface Transformers \cite{XX}, and train on a single eight-core TPU on the Google Cloud Platform.
